Rapid grain growth in post-AGB disc systems from far-infrared and sub-millimetre photometry

The timescales on which astronomical dust grows remain poorly understood, with important consequences for our understanding of processes like circumstellar disk evolution and planet formation.A number of post-asymptotic giant branch stars are found to host optically thick, dust- and gas-rich circumstellar discs in Keplerian orbits. These discs exhibit evidence of dust evolution, similar to protoplanetary discs; however since post-AGB discs have substantially shorter lifetimes than protoplanetary discs they may provide new insights on the grain-growth process. We examine a sample of post-AGB stars with discs to determine the FIR and sub-mm spectral index by homogeneously fitting a sample of data from \textit{Herschel}, the SMA and the literature. We find that grain growth to at least hundreds of micrometres is ubiquitous in these systems, and that the distribution of spectral indices is more similar to that of protoplanetary discs than debris discs. No correlation is found with the mid-infrared colours of the discs, implying that grain growth occurs independently of the disc structure in post-AGB discs. We infer that grain growth to $\sim$mm sizes must occur on timescales $<<10^{5}$ yr, perhaps by orders of magnitude, as the lifetimes of these discs are expected to be $\lesssim10^{5}$~yr and all objects have converged to the same state. This growth timescale is short compared to the results of models for protoplanetary discs including fragmentation, and may provide new constraints on the physics of grain growth.

==> floats/fluxes_old.tex <==
%\begin{landscape}
\begin{table*}%[]
    \caption{Complete list of fluxes, in Jansky}
    \centering
    \tiny
    \rotatebox{90}{
    \begin{tabular}{lccccccccc}\hline
    Source & 100 & 160 & 250 & 350 & 450 & 500 & 850 & 1300 & 3000  \\ \hline\hline
    TW Cam &--&--& 0.145 $\pm$ 0.01 & 0.074 $\pm$ 0.008 &--& 0.0 $\pm$ 0.007 & 0.011 $\pm$ 0.0023$^{a}$ &--&--\\
DY Ori & 1.431 $\pm$ 0.072 & 0.571 $\pm$ 0.032 & 0.223 $\pm$ 0.014 & 0.114 $\pm$ 0.009 &--& 0.0 $\pm$ 0.007 &--&--&--\\
CT Ori &--&--& 0.05 $\pm$ 0.008 & 0.0 $\pm$ 0.079 &--& 0.0 $\pm$ 0.056 &--&--&--\\
SU Gem & 0.819 $\pm$ 0.041 & 0.358 $\pm$ 0.022 & 0.166 $\pm$ 0.009 & 0.08 $\pm$ 0.006 &--& 0.0 $\pm$ 0.032 & 0.0075 $\pm$ 0.0025$^{a}$ &--&--\\
UY CMa & 0.136 $\pm$ 0.009 & 0.09 $\pm$ 0.012 & 0.0 $\pm$ 0.007 &--&--&--& 0.0024 $\pm$ 0.0021$^{a}$ &--&--\\
UY CMa2 & 0.162088 $\pm$ 0.011118 & 0.086943 $\pm$ 0.022655 & 0.0225 $\pm$ 0.0067 &--&--&--& 0.0024 $\pm$ 0.0021$^{a}$ &--&--\\
V382 Aur & 0.029 $\pm$ 0.005 & 0.049 $\pm$ 0.008 & 0.0 $\pm$ 0.007 &--&--&--&--&--&--\\
ST Pup & 0.362 $\pm$ 0.018 & 0.078 $\pm$ 0.009 & 0.03 $\pm$ 0.008 & 0.0 $\pm$ 0.013 &--&--&--&--&--\\
V421 CMa & 0.201 $\pm$ 0.011 & 0.029 $\pm$ 0.009 & 0.031 $\pm$ 0.008 & 0.0 $\pm$ 0.007 &--&--&--&--&--\\
U Mon & 9.12 $\pm$ 0.456 & 4.236 $\pm$ 0.212 & 2.009 $\pm$ 0.104 & 1.066 $\pm$ 0.054 &--& 0.549 $\pm$ 0.032 & 0.1816 $\pm$ 0.0026$^{a}$ & 0.1 $\pm$ 0.014$^{a}$ & 0.015 $\pm$ 0.0003$^{a}$ \\
V390 Vel &--&--& 4.229 $\pm$ 0.22 & 1.863 $\pm$ 0.097 &--& 0.588 $\pm$ 0.034 &--&--&--\\
BZ Pyx & 0.242 $\pm$ 0.013 & 0.126 $\pm$ 0.011 & 0.0 $\pm$ 0.009 &--&--&--&--&--&--\\
IRAS 09144-4933 & 1.107 $\pm$ 0.055 & 0.379 $\pm$ 0.031 & 0.0 $\pm$ 0.014 &--&--&--&--&--&--\\
IRAS 09400-4733 & 0.582 $\pm$ 0.029 & 0.27 $\pm$ 0.017 & 0.112 $\pm$ 0.007 & 0.045 $\pm$ 0.005 &--& 0.0 $\pm$ 0.007 &--&--&--\\
GP Cha & 0.163 $\pm$ 0.009 & 0.056 $\pm$ 0.009 & 0.0 $\pm$ 0.01 &--&--&--&--&--&--\\
AG Ant & 0.479 $\pm$ 0.024 & 0.235 $\pm$ 0.013 & 0.072 $\pm$ 0.008 & 0.054 $\pm$ 0.007 &--& 0.053 $\pm$ 0.009 & 0.0087 $\pm$ 0.0028$^{a}$ &--&--\\
HR 4226 &--&--& 2.158 $\pm$ 0.111 & 1.093 $\pm$ 0.058 &--& 0.53 $\pm$ 0.03 &--&--&--\\
V802 Car & 1.545 $\pm$ 0.077 & 0.983 $\pm$ 0.163 & 0.0 $\pm$ 0.014 &--&--&--&--&--&--\\
GK Car & 0.169 $\pm$ 0.011 & 0.109 $\pm$ 0.014 & 0.0 $\pm$ 0.036 &--&--&--&--&--&--\\
AF Crt & 0.321 $\pm$ 0.017 & 0.08 $\pm$ 0.01 & 0.029 $\pm$ 0.008 & 0.024 $\pm$ 0.008 &--& 0.0 $\pm$ 0.007 &--&--&--\\
RU Cen &--&--& 0.589 $\pm$ 0.031 & 0.319 $\pm$ 0.018 &--& 0.149 $\pm$ 0.012 &--&--&--\\
SX Cen &--&--& 0.083 $\pm$ 0.009 & 0.045 $\pm$ 0.008 &--& 0.0 $\pm$ 0.007 &--&--&--\\
V1123 Cen & 2.446 $\pm$ 0.122 & 0.928 $\pm$ 0.046 & 0.292 $\pm$ 0.017 & 0.126 $\pm$ 0.01 &--& 0.049 $\pm$ 0.08 &--&--&--\\
V1123 Cen2 & 2.393685 $\pm$ 0.011373 & 0.929164 $\pm$ 0.026523 & 0.295 $\pm$ 0.0152 & 0.1319 $\pm$ 0.0186 &--&--&--&--&--\\
IRAS 13258-8103 & 0.66 $\pm$ 0.033 & 0.458 $\pm$ 0.031 & 0.143 $\pm$ 0.008 & 0.051 $\pm$ 0.08 &--& 0.0 $\pm$ 0.007 &--&--&--\\
EN TrA & 1.459 $\pm$ 0.073 & 0.625 $\pm$ 0.033 & 0.266 $\pm$ 0.016 & 0.139 $\pm$ 0.01 &--& 0.075 $\pm$ 0.011 &--&--&--\\
IRAS 15469-5311 & 3.88 $\pm$ 0.194 & 1.441 $\pm$ 0.075 & 0.0 $\pm$ 0.049 &--&--&--&--&--&--\\
IRAS 15556-5444 & 2.987 $\pm$ 0.149 & 1.363 $\pm$ 0.072 & 0.66 $\pm$ 0.035 & 0.319 $\pm$ 0.018 &--& 0.169 $\pm$ 0.013 &--&--&--\\
NSV 7708 & 0.254 $\pm$ 0.013 & 0.075 $\pm$ 0.008 & 0.041 $\pm$ 0.08 & 0.0 $\pm$ 0.011 &--&--&--&--&--\\
IRAS 17038-4815 & 1.878 $\pm$ 0.094 & 0.994 $\pm$ 0.055 & 0.447 $\pm$ 0.025 & 0.268 $\pm$ 0.016 &--& 0.105 $\pm$ 0.011 &--&--&--\\
LR Sco & 0.762 $\pm$ 0.038 & 0.334 $\pm$ 0.029 & 0.086 $\pm$ 0.008 & 0.045 $\pm$ 0.006 &--& 0.06 $\pm$ 0.008 &--&--&--\\
89 Her &--&--& 0.667 $\pm$ 0.036 & 0.343 $\pm$ 0.02 &--& 0.16 $\pm$ 0.013 & 0.0409 $\pm$ 0.0024$^{a}$ & 0.0092 $\pm$ 0.0005$^{a}$ & 0.0027 $\pm$ 0.0003$^{a}$ \\
AI Sco & 1.424 $\pm$ 0.071 & 0.631 $\pm$ 0.032 & 0.301 $\pm$ 0.017 & 0.14 $\pm$ 0.009 &--& 0.068 $\pm$ 0.008 &--&--&--\\
V2053 Oph & 1.213 $\pm$ 0.061 & 0.39 $\pm$ 0.022 & 0.107 $\pm$ 0.01 & 0.032 $\pm$ 0.007 &--& 0.0 $\pm$ 0.007 &--&--&--\\
IRAS 18158-3445 & 0.375 $\pm$ 0.019 & 0.135 $\pm$ 0.011 & 1.328 $\pm$ 0.066 & 0.655 $\pm$ 0.033 &--& 0.314 $\pm$ 0.016 &--&--&--\\
AC Her &--&--& 1.572 $\pm$ 0.083 & 0.817 $\pm$ 0.044 &--& 0.38 $\pm$ 0.022 & 0.0994 $\pm$ 0.0038$^{a}$ & 0.038 $\pm$ 0.001$^{a}$ & 0.0046 $\pm$ 0.0004$^{a}$ \\
AD Aql & 0.156 $\pm$ 0.012 & 0.093 $\pm$ 0.008 & 0.035 $\pm$ 0.008 & 0.0 $\pm$ 0.007 &--&--&--&--&--\\
EP Lyr & 0.107 $\pm$ 0.007 & 0.08 $\pm$ 0.01 & 0.037 $\pm$ 0.008 & 0.026 $\pm$ 0.007 &--& 0.022 $\pm$ 0.007 &--&--&--\\
BD-02 4931 & 0.823 $\pm$ 0.041 & 0.408 $\pm$ 0.022 & 0.151 $\pm$ 0.011 & 0.093 $\pm$ 0.009 &--& 0.041 $\pm$ 0.008 &--&--&--\\
QY Sge &--&--& 0.372 $\pm$ 0.022 & 0.191 $\pm$ 0.013 &--& 0.108 $\pm$ 0.014 & 0.0218 $\pm$ 0.0018$^{a}$ &--&--\\
AR Pup &--&--& 1.597 $\pm$ 0.082 & 0.923 $\pm$ 0.052 &--& 0.443 $\pm$ 0.035 &--& 0.0416 $\pm$ 0.0021$^{z}$ &--\\
AR Pup2 &--&--& 1.5042 $\pm$ 0.22 & 0.7786 $\pm$ 0.14 &--& 0.3786 $\pm$ 0.07 &--& 0.0416 $\pm$ 0.0021$^{z}$ &--\\
AR Pup3 &--&--& 1.6104 $\pm$ 0.083 & 0.861 $\pm$ 0.096 &--& 0.4287 $\pm$ 0.0722 &--& 0.0416 $\pm$ 0.0021$^{z}$ &--\\
RV Tau & 2.414 $\pm$ 0.121 & 0.987 $\pm$ 0.049 & 0.512 $\pm$ 0.028 & 0.263 $\pm$ 0.018 &--& 0.135 $\pm$ 0.016 & 0.0503 $\pm$ 0.0036$^{a}$ & 0.015 $\pm$ 0.0008$^{z}$ & 0.0039 $\pm$ 0.0002$^{a}$ \\
RV Tau2 & 2.879379 $\pm$ 0.010871 & 1.3266 $\pm$ 0.026046 & 0.539 $\pm$ 0.0156 & 0.2923 $\pm$ 0.0153 &--& 0.1468 $\pm$ 0.014 & 0.0503 $\pm$ 0.0036$^{a}$ & 0.015 $\pm$ 0.0008$^{z}$ & 0.0039 $\pm$ 0.0002$^{a}$ \\
AY Lep & 0.68 $\pm$ 0.034 & 0.244 $\pm$ 0.012 & 0.102 $\pm$ 0.012 & 0.031 $\pm$ 0.01 &--& 0.0 $\pm$ 0.007 &--& 0.0 $\pm$ 0.001$^{z}$ &--\\
PS Gem & 0.338 $\pm$ 0.017 & 0.143 $\pm$ 0.012 & 0.075 $\pm$ 0.016 & 0.063 $\pm$ 0.015 &--& 0.024 $\pm$ 0.007 & 0.0028 $\pm$ 0.0019$^{a}$ & 0.0 $\pm$ 0.001$^{z}$ &--\\
IRAS 17233-4330 & 1.024287 $\pm$ 0.013325 & 0.496069 $\pm$ 0.029768 & 0.2782 $\pm$ 0.0409 & 0.2075 $\pm$ 0.0478 &--& 0.1322 $\pm$ 0.0338 &--&--&--\\
BD+03 3950 & 2.331153 $\pm$ 0.011126 & 0.89276 $\pm$ 0.026954 & 0.3127 $\pm$ 0.0217 & 0.1363 $\pm$ 0.0205 &--& 0.0835 $\pm$ 0.0186 &--&--&--\\
IW Car &--&--& 2.6873 $\pm$ 0.0302 & 1.4152 $\pm$ 0.0268 &--& 0.6845 $\pm$ 0.0263 & 0.2 $\pm$ 0.02$^{a}$ &--&--\\
Red Rectangle &--&--&--&--& 0.034 $\pm$ 0.002$^{b}$ &--& 0.00625 $\pm$ 0.00035$^{b}$ &--&--\\\hline
\multicolumn{10}{l}{Notes:}
\multicolumn{10}{l}{References: $a$ \citet{}; $b$ \citet{}}
    \end{tabular}
    }
    
    \label{tab:fluxes}
\end{table*}
%\end{landscape}

==> floats/mcmc_results_old.tex <==
TW Cam & -2.49835127451 $\pm^{ 0.31859633859}_{0.32524853798}$ & 0.0331863051619$\pm^{0.00526000338954}_{0.00487832671949}$& 0.00678640453324$\pm^{0.00250794444557}_{0.00193550378918}$ & 0.00235102150667$\pm^{0.00130722307337}_{0.000880601357898}$ & 0.000290824994537 $\pm^{0.000297045231474}_{0.000151304781996}$ \\
DY Ori & -3.30266614723 $\pm^{ 0.377164337383}_{0.425838546932}$ & 0.0356770784279$\pm^{0.00650762664851}_{0.00636225563708}$& 0.00437231490916$\pm^{0.00207045092157}_{0.0015775323036}$ & 0.00107808802612$\pm^{0.000776109735209}_{0.000502385604341}$ & 6.81397756895e-05 $\pm^{9.23969380597e-05}_{4.25815095294e-05}$ \\
CT Ori & -2.46393700777 $\pm^{ 1.66121177412}_{1.72189180593}$ & 0.0116762789324$\pm^{0.0205088802932}_{0.00756528779373}$& 0.00244989370341$\pm^{0.0164376684651}_{0.0021585335871}$ & 0.00086018673275$\pm^{0.0125900027412}_{0.000811288091825}$ & 0.000109646401203 $\pm^{0.00677607194983}_{0.000108177655911}$ \\
SU Gem & -2.19137957069 $\pm^{ 0.609180171419}_{0.621421188662}$ & 0.0460399702013$\pm^{0.0157744900615}_{0.0124980412525}$& 0.0114444164717$\pm^{0.0109316231042}_{0.00581767798328}$ & 0.00451335454589$\pm^{0.00688958246425}_{0.00280345505759}$ & 0.00072438579598 $\pm^{0.00229399319165}_{0.00056120954827}$ \\
%UY CMa & -2.48695891554 $\pm^{ 1.68394572596}_{1.69678727092}$ & 0.0$\pm^{4.88263163439e-155}_{0.0}$& 0.0$\pm^{1.46918128868e-155}_{0.0}$ & 0.0$\pm^{5.18557368513e-156}_{0.0}$ & 0.0 $\pm^{4.05657644692e-157}_{0.0}$ \\
UY CMa2 & -3.09812536855 $\pm^{ 1.3946843012}_{1.2783270606}$ & 0.00368673955516$\pm^{0.00497908980829}_{0.00225652496349}$& 0.000516000872799$\pm^{0.0021998414761}_{0.0004134470174}$ & 0.000137870467197$\pm^{0.00115184541652}_{0.000121289391945}$ & 1.03742805377e-05 $\pm^{0.000292073758724}_{9.93481543229e-06}$ \\
%V382 Aur & -2.48122558626 $\pm^{ 1.67784655668}_{1.71622024257}$ & 0.0$\pm^{3.36848496134e-171}_{0.0}$& 0.0$\pm^{8.7754797931e-172}_{0.0}$ & 0.0$\pm^{2.55876165559e-172}_{0.0}$ & 0.0 $\pm^{3.48363491158e-173}_{0.0}$ \\
ST Pup & -2.81844993135 $\pm^{ 1.77272081352}_{1.50420760631}$ & 0.00553374531661$\pm^{0.0094894024946}_{0.00351072543997}$& 0.000898917164001$\pm^{0.00623872285778}_{0.000756235859666}$ & 0.000270240071793$\pm^{0.00428008311918}_{0.000247247866228}$ & 2.57429044185e-05 $\pm^{0.00186557519882}_{2.51243671259e-05}$ \\
V421 CMa & -3.13925541238 $\pm^{ 1.71760905854}_{1.31360086992}$ & 0.00447644195546$\pm^{0.00585379914672}_{0.00259986784255}$& 0.000593849780473$\pm^{0.00332418492645}_{0.000471082050815}$ & 0.000155029954729$\pm^{0.00195251084635}_{0.000136112101826}$ & 1.10584492391e-05 $\pm^{0.000620367201635}_{1.05969594764e-05}$ \\
U Mon & -1.97645806006 $\pm^{ 0.0347698447804}_{0.0354038415383}$ & 0.640049483228$\pm^{0.0266920269044}_{0.025074257483}$& 0.182127049135$\pm^{0.00496517283769}_{0.00484042700417}$ & 0.078646326838$\pm^{0.00203383785196}_{0.00198881308886}$ & 0.015063201518 $\pm^{0.000651081183955}_{0.000643178028788}$ \\
V390 Vel & -2.84065777939 $\pm^{ 0.252655867715}_{0.252525742559}$ & 0.833463519932$\pm^{0.0854268396742}_{0.0778469188551}$& 0.136944040401$\pm^{0.0368735564836}_{0.0292214334848}$ & 0.0409174604582$\pm^{0.0167933068646}_{0.0119173133139}$ & 0.00379833989017 $\pm^{0.00281724536287}_{0.00160854695897}$ \\
%BZ Pyx & -2.49578457865 $\pm^{ 1.69555583932}_{1.70472425585}$ & 0.0$\pm^{2.48115491505e-153}_{0.0}$& 0.0$\pm^{4.1005411476e-154}_{0.0}$ & 0.0$\pm^{1.3859570949e-154}_{0.0}$ & 0.0 $\pm^{1.70197044532e-155}_{0.0}$ \\
%IRAS 09144-4933 & -2.48095666627 $\pm^{ 1.7060379051}_{1.70298460098}$ & 0.0$\pm^{5.16457633439e-168}_{0.0}$& 0.0$\pm^{7.73036692137e-169}_{0.0}$ & 0.0$\pm^{2.1251183819e-169}_{0.0}$ & 0.0 $\pm^{5.16753334039e-170}_{0.0}$ \\
IRAS 09400-4733 & -3.10540360728 $\pm^{ 0.62283538699}_{0.711144072406}$ & 0.0184152781305$\pm^{0.00689614967434}_{0.00561953017953}$& 0.00255099336772$\pm^{0.00261301826202}_{0.0014059455136}$ & 0.000680892355329$\pm^{0.00111107724136}_{0.000453737003166}$ & 5.07015790659e-05 $\pm^{0.000173927832485}_{4.13491733047e-05}$ \\
%GP Cha & -2.42444708052 $\pm^{ 1.66744813751}_{1.7521966195}$ & 0.0$\pm^{4.94613513888e-159}_{0.0}$& 0.0$\pm^{1.11747439634e-159}_{0.0}$ & 0.0$\pm^{4.26738153217e-160}_{0.0}$ & 0.0 $\pm^{4.72538860687e-161}_{0.0}$ \\
AG Ant & -1.13224387062 $\pm^{ 0.475493240668}_{0.486781242982}$ & 0.0401272535432$\pm^{0.00972748532216}_{0.00793002994018}$& 0.0195509977107$\pm^{0.0117209541919}_{0.00747071376492}$ & 0.0120829553888$\pm^{0.011448090751}_{0.00595215975828}$ & 0.00470474801555 $\pm^{0.00880312609543}_{0.00311719730285}$ \\
HR 4226 & -2.03145371881 $\pm^{ 0.254018297196}_{0.251628086441}$ & 0.654986887116$\pm^{0.0677553218238}_{0.0617757818627}$& 0.180040209121$\pm^{0.0485631324345}_{0.0383750932288}$ & 0.0760267390425$\pm^{0.0309810769135}_{0.0221801524396}$ & 0.0139065423714 $\pm^{0.0102286713618}_{0.00591296996342}$ \\
%V802 Car & -2.61637434363 $\pm^{ 1.74773035182}_{1.66108737785}$ & 0.0$\pm^{2.54800216288e-165}_{0.0}$& 0.0$\pm^{6.13612037924e-166}_{0.0}$ & 0.0$\pm^{2.30285634503e-166}_{0.0}$ & 0.0 $\pm^{3.71291917921e-167}_{0.0}$ \\
%GK Car & -2.42252474301 $\pm^{ 1.6619553812}_{1.71239126087}$ & 0.0$\pm^{1.01820259979e-160}_{0.0}$& 0.0$\pm^{2.16684255176e-161}_{0.0}$ & 0.0$\pm^{7.7242382937e-162}_{0.0}$ & 0.0 $\pm^{1.0852251246e-162}_{0.0}$ \\
AF Crt & -2.421712825 $\pm^{ 1.38147443361}_{1.50128508269}$ & 0.00836994729096$\pm^{0.00759240281604}_{0.00437824197514}$& 0.00181628878753$\pm^{0.0056663558876}_{0.00145383122414}$ & 0.000649349017724$\pm^{0.00402465692477}_{0.000579947123793}$ & 8.59444217683e-05 $\pm^{0.00186465260158}_{8.33043449697e-05}$ \\
RU Cen & -1.96885188771 $\pm^{ 0.312849661885}_{0.306594557482}$ & 0.187706977242$\pm^{0.026321056831}_{0.0225719997219}$& 0.0536434149254$\pm^{0.0197905117308}_{0.0141647946096}$ & 0.0232514610657$\pm^{0.0129925463382}_{0.00821428711782}$ & 0.00448341909975 $\pm^{0.00454612109837}_{0.00223550376482}$ \\
SX Cen & -2.86705320511 $\pm^{ 0.825666717581}_{0.966285122221}$ & 0.0166020157133$\pm^{0.00805569020194}_{0.00645640004095}$& 0.00269247715178$\pm^{0.00387307527539}_{0.00178626175853}$ & 0.000799388714874$\pm^{0.00193963112206}_{0.000621010437808}$ & 7.30294360004e-05 $\pm^{0.00041915148221}_{6.57515722845e-05}$ \\
V1123 Cen & -2.49962363116 $\pm^{ 0.656991140414}_{0.664532982545}$ & 0.067213308913$\pm^{0.0258519638503}_{0.0189684815853}$& 0.0136980391814$\pm^{0.014797921708}_{0.00718201192752}$ & 0.00473150205881$\pm^{0.00829129595543}_{0.00302536654221}$ & 0.000585767381137 $\pm^{0.00219500279812}_{0.000464313235912}$ \\
V1123 Cen2 & -2.3608933665 $\pm^{ 0.980494252713}_{0.996208863664}$ & 0.073615336692$\pm^{0.0536563004563}_{0.0315207600776}$& 0.0163502135435$\pm^{0.0362858585856}_{0.0113590027262}$ & 0.00599522097033$\pm^{0.0232501429735}_{0.00478882750261}$ & 0.00083439064105 $\pm^{0.00834493234083}_{0.000761283962035}$ \\
IRAS 13258-8103 & -3.91383749966 $\pm^{ 0.856574407113}_{0.727230987591}$ & 0.0143695922992$\pm^{0.00922562597683}_{0.00504700875504}$& 0.00119102637132$\pm^{0.00215852137092}_{0.000704044248259}$ & 0.000225494854336$\pm^{0.000687314928057}_{0.000157734434037}$ & 8.55096557677e-06 $\pm^{6.2271489439e-05}_{7.15063722678e-06}$ \\
EN TrA & -1.85777823053 $\pm^{ 0.451198872925}_{0.453646360846}$ & 0.0885230410905$\pm^{0.0207275231648}_{0.0162685591441}$& 0.0271927063158$\pm^{0.0167010341167}_{0.0103192518409}$ & 0.012345950569$\pm^{0.0117649170916}_{0.00599005067977}$ & 0.00260616921797 $\pm^{0.00479134234567}_{0.00168359579487}$ \\
%IRAS 15469-5311 & -2.47723716098 $\pm^{ 1.67371879425}_{1.72953296001}$ & 0.0$\pm^{7.65831692405e-163}_{0.0}$& 0.0$\pm^{1.63526248916e-163}_{0.0}$ & 0.0$\pm^{5.73492950923e-164}_{0.0}$ & 0.0 $\pm^{9.48661538739e-165}_{0.0}$ \\
IRAS 15556-5444 & -1.98690715023 $\pm^{ 0.297888875017}_{0.304759681858}$ & 0.201463347672$\pm^{0.0273525588028}_{0.0238353973599}$& 0.0569822270056$\pm^{0.0198358307897}_{0.0148378929394}$ & 0.0244568125615$\pm^{0.0129397368738}_{0.00847122778486}$ & 0.00464225422881 $\pm^{0.00445202276198}_{0.00227901839383}$ \\
%NSV 7708 & -2.52830865527 $\pm^{ 1.7167241488}_{1.64748956778}$ & 0.0$\pm^{1.37911198789e-168}_{0.0}$& 0.0$\pm^{3.24756787196e-169}_{0.0}$ & 0.0$\pm^{1.08140115079e-169}_{0.0}$ & 0.0 $\pm^{1.94957307922e-170}_{0.0}$ \\
IRAS 17038-4815 & -1.94436727077 $\pm^{ 0.365397194049}_{0.361820807515}$ & 0.149056608619$\pm^{0.0254549982098}_{0.021795104755}$& 0.043336403251$\pm^{0.0194934971129}_{0.0134574682258}$ & 0.0189691640227$\pm^{0.0130787908707}_{0.00771467023874}$ & 0.00373224218822 $\pm^{0.00479031556635}_{0.00209564024538}$ \\
LR Sco & -0.71971568407 $\pm^{ 0.425393361165}_{0.494831445878}$ & 0.0522547423859$\pm^{0.0120958195972}_{0.0104285567562}$& 0.0332098896152$\pm^{0.0180958116034}_{0.013113514272}$ & 0.024453225253$\pm^{0.0206596107865}_{0.0123970152529}$ & 0.0134194161655 $\pm^{0.0216987915582}_{0.00901485926961}$ \\
89 Her & -2.45122320865 $\pm^{ 0.081706284352}_{0.0800976953609}$ & 0.170578983142$\pm^{0.0111289613223}_{0.010543061185}$& 0.0359024385149$\pm^{0.00234726794198}_{0.00225042675079}$ & 0.0126706106739$\pm^{0.0011113162528}_{0.00103408520175}$ & 0.00163106600552 $\pm^{0.000247041933861}_{0.000214968201612}$ \\
AI Sco & -2.20629042666 $\pm^{ 0.395638933456}_{0.382030704243}$ & 0.0819214827075$\pm^{0.0155783844419}_{0.0129013154862}$& 0.020148827737$\pm^{0.0102642772073}_{0.00660226925853}$ & 0.00788417115394$\pm^{0.00616695222881}_{0.00335124868372}$ & 0.00124406832651 $\pm^{0.00184738952175}_{0.000723258269786}$ \\
V2053 Oph & -3.70524758939 $\pm^{ 0.96309473438}_{0.833018075658}$ & 0.0121813649361$\pm^{0.0081941982538}_{0.00455621310069}$& 0.00115744340498$\pm^{0.00234207383182}_{0.000726577360316}$ & 0.000239100137895$\pm^{0.000846212867061}_{0.000176154173432}$ & 1.081252545e-05 $\pm^{9.78790315057e-05}_{9.39158206884e-06}$ \\
IRAS 18158-3445 & -2.07559441824 $\pm^{ 0.237859497187}_{0.23468458797}$ & 0.391655825792$\pm^{0.0360509695749}_{0.0339058505885}$& 0.104668462483$\pm^{0.0256440344046}_{0.0209011875991}$ & 0.0433071519393$\pm^{0.0162513941964}_{0.0118108508926}$ & 0.00764345006666 $\pm^{0.00514281386926}_{0.00307395631637}$ \\
AC Her & -2.32484267069 $\pm^{ 0.0625631962361}_{0.0635111762442}$ & 0.440546352577$\pm^{0.0254039306169}_{0.0236229286649}$& 0.100470554879$\pm^{0.00408076871528}_{0.00398078288836}$ & 0.0373907591919$\pm^{0.00189204021794}_{0.00179379569718}$ & 0.00534969620441 $\pm^{0.000506493678987}_{0.000460451914734}$ \\
AD Aql & -3.14211900139 $\pm^{ 1.6484046972}_{1.2906636927}$ & 0.00489105698005$\pm^{0.00605222960988}_{0.00270226518188}$& 0.000645145097772$\pm^{0.00335696630985}_{0.000502623455277}$ & 0.00016790499719$\pm^{0.00192132829341}_{0.000145826961999}$ & 1.2056956838e-05 $\pm^{0.000581137374069}_{1.15135761319e-05}$ \\
EP Lyr & -1.23379577204 $\pm^{ 0.806114703431}_{1.04049181431}$ & 0.0192831529042$\pm^{0.0104129133872}_{0.00729346004338}$& 0.0088006814983$\pm^{0.011754018522}_{0.00572319258394}$ & 0.0052192325289$\pm^{0.011695883768}_{0.00402323370186}$ & 0.00186397514752 $\pm^{0.00980811601835}_{0.00168422328181}$ \\
BD-02 4931 & -1.70851336961 $\pm^{ 0.590939387906}_{0.583722314984}$ & 0.0563723150792$\pm^{0.0180440186515}_{0.013511679858}$& 0.0190180537469$\pm^{0.0168376062939}_{0.0088429481235}$ & 0.00921181180252$\pm^{0.0129942979225}_{0.00535412745466}$ & 0.00220904415726 $\pm^{0.00647274637731}_{0.00164126126281}$ \\
QY Sge & -2.28493807284 $\pm^{ 0.183285111156}_{0.186228637813}$ & 0.102149742617$\pm^{0.00993189884291}_{0.00907165916037}$& 0.0238257223492$\pm^{0.00459900569836}_{0.00372592319666}$ & 0.00902073429193$\pm^{0.00254549314736}_{0.00193113249498}$ & 0.00133395637962 $\pm^{0.000646498369083}_{0.000430342776279}$ \\
%AR Pup & -2.24947914436 $\pm^{ 0.0957604669344}_{0.0967458712752}$ & 0.474098716807$\pm^{0.0315496596722}_{0.0305712455687}$& 0.113262605381$\pm^{0.00973467427791}_{0.00899657010178}$ & 0.0435577316035$\pm^{0.00512318308817}_{0.00470313204331}$ & 0.00663235747278 $\pm^{0.00133962913439}_{0.00112364401156}$ \\
%AR Pup2 & -2.20567296464 $\pm^{ 0.1748966031}_{0.174820327057}$ & 0.432142967471$\pm^{0.0801683724191}_{0.0663816177624}$& 0.106339910438$\pm^{0.0120233144858}_{0.0104190405745}$ & 0.0417574426517$\pm^{0.00502723218333}_{0.0045665146805}$ & 0.00659675546504 $\pm^{0.00164708324975}_{0.00131135074002}$ \\
AR Pup3 & -2.22574227639 $\pm^{ 0.0990680640502}_{0.102808679603}$ & 0.448768219722$\pm^{0.0372921806437}_{0.0347088640532}$& 0.108843340226$\pm^{0.0100962728515}_{0.00918507830026}$ & 0.0422715894053$\pm^{0.00518893052768}_{0.00459050426286}$ & 0.00657472762859 $\pm^{0.00132180175674}_{0.00112265424258}$ \\
RV Tau & -1.99540487656 $\pm^{ 0.0623540425121}_{0.0616931605917}$ & 0.15561099416$\pm^{0.0110896419012}_{0.0104836877873}$& 0.0437236756935$\pm^{0.0026353440441}_{0.0023945256094}$ & 0.0187434325479$\pm^{0.00122684304781}_{0.00114847363275}$ & 0.00353508404657 $\pm^{0.000360444600562}_{0.000329703985076}$ \\
%RV Tau2 & -2.02906723312 $\pm^{ 0.0485414051961}_{0.0491959461972}$ & 0.164740684048$\pm^{0.00755534696824}_{0.00729099249888}$& 0.0453037679619$\pm^{0.00232758299053}_{0.00218398945724}$ & 0.019130888323$\pm^{0.00122765520487}_{0.00115528581612}$ & 0.00350601755471 $\pm^{0.000350273871383}_{0.000321377363198}$ \\
AY Lep & -3.70357877021 $\pm^{ 0.912157022852}_{0.842532301696}$ & 0.0116519495335$\pm^{0.00758119678543}_{0.00460087782447}$& 0.00110576433779$\pm^{0.00206442793662}_{0.000703312214364}$ & 0.000229910196759$\pm^{0.000731719446136}_{0.000171288917145}$ & 1.04051268684e-05 $\pm^{8.1889077196e-05}_{9.0994511874e-06}$ \\
PS Gem & -2.7545574997 $\pm^{ 0.546635235037}_{0.744431124661}$ & 0.0212276627471$\pm^{0.00795531214104}_{0.00630650269085}$& 0.00379953379461$\pm^{0.00249262185667}_{0.00196730453056}$ & 0.00119690183499$\pm^{0.00121101077526}_{0.000773196406822}$ & 0.000120547532688 $\pm^{0.000251608512235}_{9.73993243903e-05}$ \\
IRAS 17233-4330 & -1.20649207667 $\pm^{ 0.725452449681}_{0.854322934219}$ & 0.141104366138$\pm^{0.0620787037099}_{0.046170208147}$& 0.0656878099274$\pm^{0.0761466994255}_{0.0389001956541}$ & 0.0394623528468$\pm^{0.0758232563618}_{0.0281408378178}$ & 0.0144909850251 $\pm^{0.0626087064546}_{0.0124618045758}$ \\
BD+03 3950 & -2.07803821283 $\pm^{ 0.67113749068}_{0.658764970977}$ & 0.0909319889956$\pm^{0.0388987021366}_{0.0266010234359}$& 0.02423936966$\pm^{0.0279474683845}_{0.0127596697547}$ & 0.0100131045799$\pm^{0.0186210798902}_{0.00640595626224}$ & 0.00176249293016 $\pm^{0.0070505517778}_{0.00139618948657}$ \\
IW Car & -1.98469720398 $\pm^{ 0.0968334703946}_{0.0941083016904}$ & 0.841333007739$\pm^{0.0421490333706}_{0.0390793365017}$& 0.238091097081$\pm^{0.0270296960909}_{0.0236372087638}$ & 0.102432117868$\pm^{0.0163362456364}_{0.0136465773375}$ & 0.0194874969115 $\pm^{0.00500058570661}_{0.00386946186071}$ \\
Red Rectangle & -2.65743840135 $\pm^{ 0.292901681849}_{0.297225477598}$ & 0.0339138515214$\pm^{0.00505729538804}_{0.00425502791244}$& 0.00626510163607$\pm^{0.000853755215504}_{0.000760760585477}$ & 0.00202255810411$\pm^{0.000530796117956}_{0.000417710346246}$ & 0.000218939096765 $\pm^{0.000130743929015}_{8.18294287405e-05}$ \\

